Mitigation of Cyberattacks through Battery Storage for Stable Microgrid Operation

In this paper, we present a mitigation methodology that leverages battery energy storage system (BESS) resources in coordination with microgrid (MG) ancillary services to maintain power system operations during cyberattacks. The control of MG agents is achieved in a distributed fashion, and once a misbehaving agent is detected, the MG's mode supervisory controller (MSC) isolates the compromised agent and initiates self-healing procedures to support the power demand and restore the compromised agent. Our results demonstrate the practicality of the proposed attack mitigation strategy and how grid resilience can be improved using BESS synergies. Simulations are performed on a modified version of the Canadian urban benchmark distribution model.

==> old_tex_files/Introduction.tex <==
\section{Introduction} \label{s:Introduction}

% powergrids blah blah
In the last decades, the power grid has undergone significant overhauls. Bulk coal-based generation plants have been replaced by economically viable distributed generation architectures which minimize the environmental footprint. Microgrids, demand-response schemes, day-ahead markets, etc.  support the provision of flexible energy to consumers and loads, overcoming the overheads of sourcing centrally generated energy from geographically dispersed facilities. Inverter-based resources and battery energy storage systems (BESS) have significantly contributed to this end, provisioning locally generated power while alleviating power consumption hot-spots (e.g., city centers) supporting peak-shaving mechanisms.

% motivation and cyberattack threat vectors
On the flip-side, the shocking rate at which new technologies, such as communication and information technologies, have been incorporated into power systems to harness the advantages of these newly deployed distributed generations (DGs) arises security concerns. The socio-economic aspects of power supply interruptions render the power grid a prominent target for cyber-attacks. The power grid's diverse and interoperable nature expands the threat landscape, while even sophisticated security architectures are bound to suffer from vulnerabilities (e.g., zero-days) given that the cyber-attacks targeting critical infrastructures are increasing. In light of such information, it is crucial to realize security mechanisms that can effectively detect malicious grid behavior and leverage the power grid's resources to overcome such adverse phenomena.

% types of attacks & attackers
In the literature diverse cyber-attack types targeting the different layers of power grid systems -- with varying degrees of impact -- have been explored \cite{zografopoulos2021cyber}. From a conservative standpoint, determined adversaries with sufficient resources (e.g., state-funded actors) can mount their attacks on multiple grid components or even coordinate sophisticated attack chains maximizing the attack impact. 

For instance, attacks could target the communication fabric between DGs (e.g., communication protocols), delaying, deleting or modifying packages (Dolev Yao adversary model) causing denial-of-service attacks \cite{zografopoulos2020derauth}. On the other hand, attackers which have achieved persistence on DG resources, could modify the firmware of inverter-based resources causing uneconomic or intermittent operation and triggering blackouts causing failures and jeopardizing grid equipment \cite{kuruvila2021hardware, zografopoulos2021security}. Granted that experimenting on real systems can be either costly or unfeasible, cyber-physical testbeds are ideal for power system security evaluation, implementation of control algorithms, and experimentation purposes. Furthermore, cyber-physical testbeds can help account for the diversity of power systems, evaluate the performance of security countermeasures, and develop practical mitigation techniques leveraging system resources, i.e., BESS.


%%%%%%%%%%%%%%%%%% Related Work %%%%%%%%%%%%%%%%%%%

However, relying solely on security mechanisms to deal with cyber-attacks targeting critical infrastructure is not a panacea. To harden power systems against adversaries, compound security and intrusion-tolerant mechanisms that can detect anomalous behavior and proactively perform remediation actions leveraging system resources need to be automated \cite{bessani2008crutial}. The importance of system resources, such as BESS, in supporting ancillary power grid services is discussed in \cite{li2019review}. Different scenarios are presented where BESS can be used to minimize power fluctuations, regulate grid voltage and frequency, optimize power flows and support distributed systems under cyber-attacks or other unexpected conditions. In \cite{6194234}, the authors present an algorithm that can coordinate the distributed energy resource (DER) contribution of multiple assets when supporting power grids. The interconnected DERs coordinate in a distributed manner and based on their capacities, contribute active and reactive power flows and injections enhancing the system stability. 

Control strategies have also been employed to maintain security and resiliency in power systems architectures. For instance, a resilient and distributed control strategy -- leveraging power sharing between multiple energy storage resources -- to regulate the frequency and voltage in autonomous MGs is proposed in \cite{9039721}. A resilient controller for multiagent systems under sensor and actuator attacks is presented in \cite{8439042}. The control schemes operate following the leader-follower scheme where the leader indicates the objectives that the follower agents should track. To mitigate the impact that compromised agents can have on the overall system, a confidence score is utilized for the agents allocating weights to the exchanged information and removing untrustworthy agent data from the system. 

Similarly, two distributed control strategies utilizing a consensus-based leader-follower approach are demonstrated in \cite{sharma2017agent}. In both schemes, the agents' behavior is monitored for malicious actions and a linear quadratic regulator problem is defined to ensure the optimal power exchange between multiple energy storage resources. The proposed schemes enable the recovery of compromised agents and allow the agents to converge to  their nominal states. Distributed control methodologies have also been used to detect and mitigate of DoS attacks targeting grid communications. In \cite{ding2019distributed} the authors demonstrate 
an acknowledgment-based detection algorithm that serves as the preliminary step before recovering the compromised grid agents. However, the successful agent recovery is contingent upon the capability of the BESS to support power demand and meet the operation and transient constraints of power systems. To achieve this goal, an adapted secondary control scheme is proposed maintaining the frequency within acceptable limits.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The contribution of this work aims to leverage both aforementioned verticals, i.e., control and BESS resource allocation, and provide an automated and resilient methodology for the detection of maliciously operating DG agents in a MG setup. By isolating the affected DGs, their behavior can be detained safeguarding the operation of the rest of the grid. Then, leveraging the BESS resources, the power demand of the compromised (islanded DG) can be supplied while the MG system operator attempts to re-actively restore the misbehaving agent to an trusted operating condition.


The rest of the paper is structured as follows. Section \ref{s:systemModel} presents the cyber and physical system modeling of this work. Section \ref{s:Methodology} details the attack preliminaries and describes the cyber-attack mitigation methodology leveraging BESS resources, while Section \ref{s:results} provides the experimental evaluation of our approach. Last, Section \ref{s:Conclusion} concludes the paper and provides directions for future work.

==> old_tex_files/Methodology.tex <==
\section{Methodology} \label{s:Methodology}
In this section, we will define the adversarial capabilities in addition to the attack assumptions and specifics for our use case. We detail the formalization for the leader-follower distributed control scheme and provide the constraints for the BESS nominal operation. Last, we discuss our malicious agent detection methodology and designate the steps of our proposed BESS-assisted MG self-healing mechanism. 

\subsection{Adversary and Attack Model}
It is assumed that the adversary could conduct attacks on the communication layer dispatching incorrect measurements to deceive the surrounding nodes. The actual measurement $y$ changes to $y^{a}$ once the vulnerability of the communication between the targeted node and its neighboring nodes is exploited. Since the relationship between the received measurement ($\widetilde{y}$) and the control signal ($u$) can be generally expressed in Eq.(\ref{eq:attacky}), where $H$ is a feedback control gain \cite{zhou2020secure}. Therefore, when
the controller takes the malicious measurement $y^{a}$ instead of the true measurement $y$, where $\widetilde{y} = y^{a}$, the control scheme is misled by the attacker.    



\begin{equation}
    u(t) = -H \widetilde{y}(t)
 \label{eq:attacky}   
\end{equation}

To establish such attacks against the measurement signal, several attack models \cite{mohan2020comprehensive} can be utilized by the adversary. The attacked measurement is described by $y^{a}_{t}$, $y_t$ is the true measurement, and the attack duration is from $t_{a}$ to $ t_{a'}$.  


\subsubsection{The scaling attack} 

This type of attack could increase or reduce $a_s+1$ times measurement to the actual measurement value by using the scaling attack vector $a_s$ as shown in Eq.(\ref{eq:attackca}). 

\begin{equation}
y^{a}_{t}=\left\{\begin{array}{ll}
y_{t} & \text { for } \mathrm{t} \notin [t_{a}, t_{a'}] \\
\left(1+a_{s}\right) y_{t}& \text { for } \mathrm{t} \in [t_{a}, t_{a'}]
\end{array}\right.
\label{eq:attackca} 
\end{equation}


\subsubsection{The additive attack}
It adds an additive attack vector $a_a$ on the original measurement during the attack period as formulated in Eq.(\ref{eq:attackaa}).  

\begin{equation}
y^{a}_{t}=\left\{\begin{array}{ll}
y_{t} & \text { for } \mathrm{t} \notin [t_{a}, t_{a'}] \\
y_{t} + {a_{a}} & \text { for } \mathrm{t} \in [t_{a}, t_{a'}]
\end{array}\right.
\label{eq:attackaa} 
\end{equation}


\subsubsection{The ramping attack}
The ramping attack vector $a_r$ is gradually modified the actual measurement with time during attack which can be modeled as below Eq.(\ref{eq:attackra}): 

\begin{equation}
y^{a}_{t}=\left\{\begin{array}{ll}
y_{t} & \text { for } \mathrm{t} \notin [t_{a}, t_{a'}] \\
y_{t} + {a_{r}} t & \text { for } \mathrm{t} \in [t_{a}, t_{a'}]
\end{array}\right.
\label{eq:attackra} 
\end{equation}

Other than the attack model, there are two ways to inject the signal of such attacks. The constant signal is considered as a one-time attack, where the attacker implements the attack in a specific instant (e.g., $[t_{a}, t_{a'}]$). Another one is called periodic signal, where the attacker injects the malicious vectors repeatedly within a period $T$ (e.g., $ [T+t_{a}, T+ t_{a'}]$). More specifically, When the information is transferred between the nodes through the cyber layer, the active power and reactive power of the neighboring converters can be manipulated. The primary droop control scheme can be deceived if malicious measurements are considered. Therefore, the system frequency and voltage stability are disturbed directly via droop control with  incorrect (manipulated) measurements.   



\subsection{Distributed Control for Agent Systems} \label{distributed_control}

Leveraging the cyber modeling formalization presented in Section \ref{cyberLayer}, we have opted for a leader-follower based consensus scheme to harden the control of MG agents in the presence of stealthy adversaries  \cite{sharma2017agent}. In such a hybrid distributed control system, the distributed agents' (i.e., DGs) objective is to track the state of the leader. The control objective at time $t$ for the $i^{th}$ agent in such leader-based distributed control system is described by Eq. \eqref{eq:DCA} \cite{sharma2017agent}.

\begin{equation}
\begin{aligned}
    u_{i}(t)=-h_{i}(t) \sum_{j=1, i\neq j}^{n} & \alpha_{ij}(t)(x_{i}(t) - x_{j}(t)) \\
    &- h_{i}(t)b_{i}(x_{i}(t) - x_{0}(t))\\
\end{aligned}
\label{eq:DCA}
\end{equation}

Where $x_{i}(t)$, $ u_{i}(t)$, and $\alpha_{ij}(t)$ are the state information, the control input, and the element of the adjacency matrix $A$ for the $i^{th}$ agent at time $t$. Agent $0$ is the leader and its corresponding state that the rest of the agents need to track is $x_{0}(t)$.  $h_{i}(t)$ is the local control gain and $b_{i}$ is equal to $1$ if the control information originates from the leader, else it is $0$. In leader--follower distributed control schemes the DG LCs are responsible to track the operational system state as indicated by the leader. As a result, to attain consensus between all system nodes Eq. \eqref{eq:consensus} needs to be satisfied.

\begin{equation}
\begin{aligned}
\label{eq:consensus}
    \lim_{t \to \infty}  |x_{i}(t) - x_{0}(t)| = 0
\end{aligned}
\end{equation}

\subsection{Microgrid Recovery Mechanism using Energy Storage}

In our case, the leader of the MG system is the MSC. The MSC monitors and supervises the nominal operation of the system by issuing control commands to the DG agents, enforcing the economic operation, managing the BESS resources (placed on the PCC) and providing remediation actions in case of adverse events. For instance, after the detection of a misbehaving agent, the leader will issue a disconnect command to the circuit breaker (CB) of the aforementioned agent and at the same time instruct the remaining DG agents to remove the node from their consensus set. Recovery of the compromised agent will then be initiated with coordination between the affected node and the MSC. Leveraging the BESS energy reserves the MSC will attempt the recovery of the maloperating DGs in accordance with the secondary frequency control constraints (Eq. \eqref{eq:Droop2}). The automatic recovery of the abnormally operating DGs can be performed -- as will be presented in Section \ref{s:results} -- granted that Eq. \eqref{eq:bessPow} - \eqref{eq:bessFreq} are true.

\begin{equation}
\begin{aligned}
\label{eq:bessPow}
   P_{BESS}^{min} \leq P_{BESS}(t) \leq P_{BESS}^{max} 
\end{aligned}
\end{equation}
\vspace{-5mm}
\begin{equation}
\begin{aligned}
\label{eq:bessSOC}
    SOC_{limit}^{min} \leq SOC_{BESS}(t) \leq SOC_{limit}^{max} \; , \forall \; t
\end{aligned}
\end{equation}

Where $P_{BESS}^{min}$ and $ P_{BESS}^{max} $ are the minimum and maximum limits of power that the BESS can supply, and $SOC_{limit}^{min}$ and $SOC_{limit}^{max}$ describe the state of charge (SOC) range within which the BESS should be operated. 

\begin{equation}
\begin{aligned}
\label{eq:bessFreq}
    \lim_{t \to t+t_{lim}} = |\omega_{BESS}(t) - \omega_{ref}| = 0  \\
    \omega_{BESS}(t) = \omega_{ref} \; , \;
    \forall \; t \geq t+t_{lim}
\end{aligned}
\end{equation}

Furthermore, the frequency of the DG when supported by the BESS ($\omega_{BESS}(t)$) should be regulated to the reference frequency $\omega_{ref}$ within the system settling timing constraint $t_{lim}$.

\subsection{Malicious Agent Behavior Mitigation }

In the event of a cyberattack or an arbitrary fault condition, one or more agents might start operating erroneously. Fault conditions are efficiently detected since they violate the system semantics in a congruent way and automated mitigations to overcome such diverse effects are built in power systems. On the other hand, a cyber-attack will manipulate an agent's operation in ``indistinguishable from normal'' way, by poisoning the information it shares with other agents, causing communication delays, blocking the information exchanged between agents, corrupting the control inputs to the underlying LC devices (within the DG), etc. By propagating the compromised information to the rest of the agents the distributed control scheme can also be corrupted %leading to uneconomic operation and 
jeopardizing the efficient operation of the whole MG. For instance, the state information of the compromised $i^{th}$ agent can be described using Eq. \eqref{eq:DCA} as follows.

\begin{equation}
\begin{aligned}
\label{eq:state}
    x_{i}(t+1) = x_{i}(t) + u_{i}(t)
\end{aligned}
\end{equation}

Where $ u_{i}(t) = - h_{i} \widetilde{y}_{i}(t)$ (Eq. \eqref{eq:attacky}) includes the attacked measurement components under scaling, additive, or ramping attacks.

It is crucial for the MG system operation to detect and mitigate the effects of maliciously operating agents before their attacks become crippling for the system. For the detection of such conditions, different approaches have been pursued. Related works leverage acknowledgement-based messages exchanged between the nodes which should arrive within predefined time limits to verify nominal agent behavior \cite{ding2019distributed, sharma2017agent}. Other approaches utilize anomaly detection, or reputation-based schemes to detect misbehaving agents \cite{zeng2014reputation, wan2017double}.

Our methodology builds on the leader-follower control mechanism and leverages the information exchanged between the DG agents and the MSC to identify suspicious behavior. We utilize a threshold-based approach where the cyber-physical properties of the system, i.e., state information ${x}=\left[ \beta, v_{od}, v_{oq}, i_{od}, i_{oq}, i_{d}, i_{q}, P_{G}, Q_{G}, \omega, V \right]^{T}$ along with the DG inverter's controller settling time, the total harmonic distortion (THD), etc.,  can signal abnormal operation. The operational thresholds for such properties in the attack-free case are well-defined \hl{need ref here}. However during malicious operation, such as during scaling, additive, or ramping attacks,  the state residuals of the compromised agents diverge from their expected values as can be seen in Fig. \hl{put label here}. 

Once abnormal agent behavior is identified, the MSC immediately issues an islanding command disconnecting the attacked DG from the system detaining the attack propagation to the rest of the DGs. Once the DG is isolated, i.e. in autonomous mode, the MSC will attempt its recovery. The self-healing process can either be performed in coordination with the DG unit -- if the controller has the ability to overcome the attack -- or in a supervisory mode. In the latter case, which is presented in this work, the MSC (leader) will decouple the compromised generation unit (e.g., the inverter within the DG), and utilize the available BESS resources to supply the power demand of the DG. Granted that the BESS can support the corresponding power demand (Eqs. \eqref{eq:bessPow}, \eqref{eq:bessSOC}, \eqref{eq:bessFreq} are satisfied) the agent will be seamlessly reconnected with the rest of the system. Once the agent reconnection has succeeded, the MSC will attempt a black-start, i.e., rebooting and restoring the DG inverter controller to a safe operational mode\cite{lopes2005control}. The algorithm of the BESS assisted MG self-healing process is outlined in Alg. \ref{alg:healing}.



\begin{algorithm}[t]
\setstretch{1}
\small
\SetAlgoLined
\DontPrintSemicolon
\textbf{Input} DG agent \emph{Data}, BESS \emph{state} \\
\textbf{\#define} int {\it $\tau$}   \\
initialize.MG(read.Agent(\emph{Data})) \\
 \While{ MG.MSC(enabled) }{
     \For {a \textbf{in} \emph{Agents} }
        {
          \If{a.stateInfo() $\geq$ {\it $\tau$} }{ 
                a.CircuitBreaker.disconnect() \Comment{Attacked agent}  \\
                a.status = OFF \\
                
                \If{BESS.state() $==$ valid  }{ 
                    \emph{\# Support demand via BESS } \\
                    a.InverterController.disconnect() \\
                    BESS.supportDemand() \\
                    a.CircuitBreaker.connect() \\
                    a.InverterController.reboot()
                }
          }
        } 
        % \emph{\# Rejuvenate compromised agents}\\
        \For {a \textbf{in} \emph{Agents.status $==$ OFF} }
        {
          \If{a.stateInfo() $\leq$ {\it $\tau$}  }{ 
                a.status = ON \Comment{Regenerate agent} \\
                a.InverterController.connect() \\
                BESS.disconnect() \\
          }
        } 
}
\vspace{-1mm}
\caption{MG self-healing mechanism.}
\label{alg:healing}
\end{algorithm}



==> old_tex_files/systemmodel.tex <==
\section{Microgrid model and Control Objectives} \label{s:systemModel}

\begin{figure}[t]
\centerline{\includegraphics[width=0.34\textwidth]{Figs/model.PNG}}
\caption{The structure of the microgrid (MG) with physical layer (black lines) and cyber layer (blue lines) of Canadian urban benchmark distribution system.}
\label{fig:architecture}
\end{figure}

Centralized, decentralized, and distributed control schemes are known as the three commonly used control approaches in MGs \cite{mirafzal2020grid,d2020towards}. Although centralized control can monitor the entire system operation and realize an accurate power sharing between converters, the communication burden limits its application to large-scale systems. However, the decentralized control can achieve  a solitary control only depending on the local information. Compared to the two former approaches, the distributed control reduces the overall communication dependency by utilizing the localized information collected from its neighboring nodes. 


\subsection{Cyber Layer Modeling} \label{cyberLayer}

Distributed control schemes utilize peer-to-peer communication between its neighboring nodes via sparse distributed communication networks. The communication network can be formulated by $G = (V, E )$, where $V=\left \{ {v_{1}, v_{2}, ....., v_{n} }\right \}$ refers to a set of $n$ nodes, and $E  \subseteq V \times V $ is a set of edges. If $e _{ij} = e_{ji}= (i, j)\in  E $, the nodes $i$ and $j$ are adjacent, which can exchange information through the communication network between them. Taking consideration of $n$ nodes and the corresponding communication network (i.e., edges), an adjacency matrix $A = [a_{ij}]$ can be obtained. $a_{ij}$ = 1 when two nodes are neighboring, otherwise $a_{ij}$ = 0. The neighboring set of a node $i$ can be written as $N_{i} = \left \{ j\in  V| e_{ij} \in  E  \right \} $. 


A modified version of the Canadian urban benchmark distribution system is utilized to demonstrate the leader-follower distributed control scheme as shown in Fig. \ref{fig:architecture} with the blue color. It is assumed that each converter has a local controller (LC), operating under a distributed control scheme. The information $\left \{ P, Q \right \}$ is exchanged between neighboring nodes to achieve primary control objectives, where $P,Q$ are the active and reactive power sharing. For example, LC2 communicates and collects the information from LC1 and LC3, which can be represented as LC2=$\left \{\xi_{12}, \xi_{32}\right \}$, where $\xi_{12} =\left \{{P_{1},Q_{1}}\right \}$ and $\xi_{32} =\left \{{P_{3},Q_{3}}\right \}$ are the information collected from LC1 and LC3 and transferred to LC2 respectively. Furthermore, a mode supervisory controller (MSC) is placed close to the point of grid connection, which can multicast signals to the respective LCs, realizing the secondary control objectives.


\subsection{Physical Layer Modeling}

DGs can be integrated into an AC MG through power converters. When the MG is connected to the main grid, known as the grid-tied mode, the converters perform as current sources. The MG voltage and frequency is mainly regulated by the main grid. Otherwise, when the MG is disconnected from the main grid, known as the grid-forming or islanded mode, it will be stablized by the converters which can operate in voltage-source or current-source mode. The modeling of strong MGs in grid-forming mode will be investigated in this work considering potential vulnerabilities against cyber-attacks and methods to mitigate using BESS planning. The droop control strategy is widely utilized to share power among parallel-connected converters and improve system reliability by imitating the parallel operation behavior of synchronous generators. Besides, it is referred to as the independent, autonomous, and wireless control due to elimination of intercommunication links between the converters. 



%  \subsubsection{Grid forming mode}
To model the system, we assume that there are $n$ nodes consisting of loads and DGs (e.g., renewable energy sources or energy storage systems). The complex power delivered to the MG from the converter on node $i$ can be calculated by $ S=V_{\mathrm{g}} I^{*}_{o i}$, where $V_\mathrm{g}\angle 0$ represents the grid voltage and $I_{o}$ is the current injected into the grid. Thus, the converter active and reactive power output can be expressed as Eq. (\ref{eq:pq}), where $V_{{i}}\angle \beta_{i}$ is the converter output voltage and $Z_{i}\angle \theta_{i}$ represents the output filter and line lumped impedance between the converter and grid.



% $\left\{\begin{array}{l}P=\frac{V_{\mathrm{com}} E}{Z} \cos (\theta-\delta)-\frac{V_{\mathrm{com}}^{2}}{Z} \cos (\theta) \\ Q=\frac{V_{\mathrm{com}} E}{Z} \sin (\theta-\delta)-\frac{V_{\mathrm{com}}^{2}}{Z} \sin (\theta)\end{array}\right.$

\begin{equation}
\left\{\begin{array}{l}P_{G i}=\frac{V_{\mathrm{g}}V_{\mathrm{i}}}{Z_{i}} \cos (\theta_{i}-\beta_{i})-\frac{V_{\mathrm{g}}^{2}}{Z_{i}} \cos (\theta_{i}) \\ Q_{G i}=\frac{V_{\mathrm{g}} V_{\mathrm{i}}}{Z_{i}} \sin (\theta_{i}-\beta_{i})-\frac{V_{\mathrm{g}}^{2}}{Z_{i}} \sin (\theta_{i})
\end{array}\right.
\label{eq:pq}
\end{equation}
 


% $$
% S=V_{\mathrm{com}} I^{*}=\frac{V_{\mathrm{com}} E \angle \theta-\delta}{Z}-\frac{V_{\mathrm{com}}^{2} \angle \theta}{Z}
% $$
% ch the real and reactive powers are achieved as
% $\left\{\begin{array}{l}P=\frac{V_{\mathrm{com}} E}{Z} \cos (\theta-\delta)-\frac{V_{\mathrm{com}}^{2}}{Z} \cos (\theta) \\ Q=\frac{V_{\mathrm{com}} E}{Z} \sin (\theta-\delta)-\frac{V_{\mathrm{com}}^{2}}{Z} \sin (\theta)\end{array}\right.$
% ective line impedance, $Z \angle \theta$, is assumed to be $\theta=90^{\circ},$ then (2) can be reduced to
% $$
% \left\{\begin{aligned}
% P &=\frac{V_{\mathrm{com}} E}{Z} \sin \delta \\
% Q &=\frac{V_{\mathrm{com}} E \cos \delta-V_{\mathrm{com}}^{2}}{Z}
% \end{aligned}\right.
% $$

When the phase difference is small enough and impedance $Z\angle \theta$ is assumed to be purely inductive with $\theta=90^{\circ}$. The $P-\omega$ and $Q-V$ droop control characteristic, {also known as primary control,} can be described by Eq.(\ref{eq:Droop1}), where $\omega$ and  $V$ are the angular frequency and converter output voltage of the inverter, $\omega_{0}$ and $V_{0}$ are the the angular frequency and converter voltage when there is no load, $k_{P}$ and $k_{Q}$ are the droop coefficients. 
 
% \begin{equation}
% \begin{aligned}
% P_{0}-k_{p}\left(\omega_{m}-\omega_{0}\right)-P_{\mathrm{out}}=J \omega_{m} \frac{d \omega_{m}}{d t}+D\left(\omega_{m}-\omega_{g}\right)
% \label{eq:Droop}
% \end{aligned}
% \end{equation}


% $P_{0}-P_{\mathrm{out}}= k_{p} (\omega_{m}-\omega_{0})$. 
 
\begin{equation}
\begin{aligned}
% f_{i} &= f_{set} + m_{i} \cdot \Delta {P}\\
% % v_{i} &= v_{set} + v_{i} \cdot \Delta {Q}\\
\omega = \omega_{0} - k_{P} \cdot P_{G} \\
V = V_{0} - k_{Q} \cdot Q_{G} 
\end{aligned}
\label{eq:Droop1}
\end{equation}


Although the droop control can achieve independent active and reactive power control in the primary level or converter level without intercommunication between nodes, it is still recommend to adopt a secondary level or system level control to compensate the frequency and voltage deviation caused by the primary level droop control operation. {Especially in the distributed control scheme under investigation, the secondary level control takes the voltage ($V_{s}$) and frequency ($\omega_{s}$) of the PCC point. Ultimately, the droop control can be formulated as Eq.(\ref{eq:Droop2}), where $\Delta \omega $ and $\Delta V$ are the secondary frequency and voltage contribution respectively.} 


% The secondary control usually compensates the error introduced by the droop coefficient 
\begin{equation}
\begin{aligned}
% f_{i} &= f_{set} + m_{i} \cdot \Delta {P}\\
% % v_{i} &= v_{set} + v_{i} \cdot \Delta {Q}\\
\omega = \omega_{0} - k_{P} \cdot P_{G} +\Delta \omega \\
V = V_{0} - k_{Q} \cdot Q_{G} + \Delta V 
\end{aligned}
\label{eq:Droop2}
\end{equation}


\begin{figure}[t]
\centerline{\includegraphics[width=0.4\textwidth]{Figs/control.PNG}}
\caption{The control mechanism of the converters. \hl{should we keep it?}}
\label{fig:control}
\end{figure}


\begin{comment}

In order to approximate the behavior of electronic circuits of the converter, small-signal model is utilized to construct linear equations for the nonlinear components in the system. The dynamic feature of the current and voltage can be modeled as below \cite{mohamed2008adaptive} : 

\begin{equation}
\begin{array}{c}
\frac{d i_{\mathrm{d}}}{d t}=\frac{-R_{f}}{L_{f}} i_{d}+\omega_{\mathrm{o}} i_{q}+\frac{1}{L_{f}}\left(v_{d}-v_{\mathrm{od}}\right) \\
\frac{d i_{\mathrm{q}}}{d t}=\frac{-R_{f}}{L_{f}} i_{q}-\omega_{\mathrm{o}} i_{d}+\frac{1}{L_{f}}\left(v_{q}-v_{\mathrm{o} q}\right) \\
\frac{d v_{\mathrm{od}}}{d t}=\omega_{\mathrm{o}} v_{\mathrm{oq}}+\frac{1}{C_{f}}\left(i_{d}-i_{\mathrm{od}}\right) \\
\frac{d v_{\mathrm{oq}}}{d t}=-\omega_{\mathrm{o}} v_{\mathrm{od}}+\frac{1}{C_{f}}\left(i_{q}-i_{\mathrm{oq}}\right) \\
\frac{d i_{\mathrm{od}}}{d t}=\frac{-R_{c}}{L_{c}} i_{\mathrm{od}}+\omega_{\mathrm{o}} i_{\mathrm{oq}}+\frac{1}{L_{c}}\left(v_{\mathrm{od}}-v_{s d}\right) \\
\frac{d i_{\mathrm{oq}}}{d t}=\frac{-R_{c}}{L_{c}} i_{\mathrm{oq}}-\omega_{\mathrm{o}} i_{\mathrm{od}}+\frac{1}{L_{c}}\left(v_{\mathrm{oq}}-v_{s q}\right)
 \label{eq:smalls}
\end{array}
\end{equation}

where $i_{\mathrm{d}}$, $i_{\mathrm{q}}$, $v_{\mathrm{d}}$, $v_{\mathrm{q}}$ are the d- and q-axis currents and voltages of the converter. $i_{\mathrm{od}}$, $i_{\mathrm{oq}}$, $v_{\mathrm{od}}$, $v_{\mathrm{oq}}$ are the d- and q-axis output currents and voltages of the converter, $v_{\mathrm{sd}}$, $v_{\mathrm{sq}}$ are the d- and q-axis bus voltages, $R_{\mathrm{f}}$, $L_{\mathrm{f}}$, $c_{\mathrm{f}}$ are the resistance, inductance, and capacitance of the $LC$ filter at each phase,  $R_{\mathrm{c}}$, $L_{\mathrm{c}}$ are the  resistance and inductance of the coupling inductor at each phase. 

\end{comment}

% By utilizing  d- and q-axis output currents and voltages of the converter, the instantaneous active $p$ and reactive power $q$ injected to the grid can be formulated as Eq.(\ref{eq:pqss}).

% It can be further used to calculate the the average active $P_{G}$ and reactive powers $P_{G}$ as Eq.(\ref{eq:PQ}).


% \begin{equation}
% \begin{array}{l}
% p=v_{\mathrm{od}} i_{\mathrm{od}}+v_{\mathrm{oq}} i_{\mathrm{o} q} \\
% q=v_{\mathrm{od}} i_{\mathrm{oq}}-v_{\mathrm{oq}} i_{\mathrm{od}}
% \label{eq:pqss}
% \end{array}
% \end{equation}



% \begin{equation}
% \begin{aligned}
% P_{G} &=\frac{\omega_{c}}{s+\omega_{c}} p \\
% Q_{G} &=\frac{\omega_{c}}{s+\omega_{c}} q
% \label{eq:PQ}
% \end{aligned}
% \end{equation}


In terms of Eq.(\ref{eq:pq}) - Eq.(\ref{eq:Droop2}), a converter can be linearized as the following state-space model in Eq.(\ref{eq:pgm}) with $a$ inputs, $b$ states, and $c$ outputs. The state derivatives $ \dot x \in \mathbb{R}^{b} $ is calculated using the state variables $x \in \mathbb{R}^{b} $ at time $t$ and system control input $u \in \mathbb{R}^{a}$. $y \in \mathbb{R}^{c}$ is the system output (sensor measurement). $A \in \mathbb{R}^{b\times b}$, $ B\in \mathbb{R}^{b \times a}$, $ C\in \mathbb{R}^{c \times b}$ are the state, control and output matrices of the physical system respectively, and $e$ denotes the noise of senor measurement. 



\begin{equation}
\begin{aligned}
 \dot{{x}}_{t} &= A x_{t} + B u_{t}\\
 {y}_{t} &= C x_{t} + e_{t}
\end{aligned}
\label{eq:pgm}
\end{equation}

Where the state variable $x_{t}$ and control input $u_{t}$ are expressed in Eq.(\ref{eq:xandu}).  

\begin{equation}
\begin{aligned}
{x}&=\left[ \beta, v_{od}, v_{oq}, i_{od}, i_{oq}, i_{d}, i_{q}, P_{G}, Q_{G}, \omega, V \right]^{T}\\
{u}&=\left[{\omega_\mathrm{s}},{V_\mathrm{s}}\right]^{T}
\label{eq:xandu}
\end{aligned}
\end{equation}



%  P_{\text {ref}} , Q_{\text {ref}}


% The local control input of the secondary controller is defined as shown in Eq.(\ref{eq:Dcontrol}) by differentiating the Eq.(\ref{eq:Droop}), where $x$ is the state variable of the system 

% \begin{equation}
%     u_{i}(t) = \sum_{j\in N} a_{ij} (x_{j}(t)-x_{i}(t))
% \label{eq:Dcontrol}
% \end{equation}



% The frequency restoration control input can be compromised by adversarial based on Eq.(\ref{eq:attacku}). 


\begin{comment}

\subsection{Attack Model}

It is assumed that the adversary could conduct attack on the communication layer which dispatching the incorrect measurements to deceive the surrounding nodes. The actual measurement $y$ changes to $y^{a}$ once the vulnerability of the communication between the targeted node and its neighboring nodes is exploited. Since the relationship between the received measurement ($\widetilde{y}$) and the control signal ($u$) can be generally expressed in Eq.(\ref{eq:attacky}), where $H$ is a feedback control gain \cite{zhou2020secure}. Therefore, when
the controller takes the malicious measurement $y^{a}$ instead of the true measurement $y$, where $\widetilde{y} = y^{a}$, the control scheme is misled by the attacker.    



\begin{equation}
    u(t) = -H \widetilde{y}(t)
 \label{eq:attacky}   
\end{equation}




% . Therefore, the state variable under attacked $x^{a}$ as shown in Eq.(\ref{eq:attackx}) with a injected attack vector $x^{a}$. 

% \begin{equation}
%     x^{a}(t) = x(t) + x^{a}
%  \label{eq:attackx}   
% \end{equation}

In order to establish such attacks against the measurement signal, several attack models \cite{mohan2020comprehensive} can be utilized by the adversary. The attacked measurement is described by $y^{a}_{t}$, $y_t$ is the true measurement, and the attack duration is from $t_{a}$ to $ t_{a'}$.  


\subsubsection{The scaling attack} 

This type of attack could increase or reduce $a_s+1$ times measurement to the actual measurement value by using the scaling attack vector $a_s$ as shown in Eq.(\ref{eq:attackca}). 

\begin{equation}
y^{a}_{t}=\left\{\begin{array}{ll}
y_{t} & \text { for } \mathrm{t} \notin [t_{a}, t_{a'}] \\
\left(1+a_{s}\right) y_{t}& \text { for } \mathrm{t} \in [t_{a}, t_{a'}]
\end{array}\right.
\label{eq:attackca} 
\end{equation}


\subsubsection{The additive attack}
It adds an additive attack vector $a_a$ on the original measurement during the attack period as formulated in Eq.(\ref{eq:attackaa}).  

\begin{equation}
y^{a}_{t}=\left\{\begin{array}{ll}
y_{t} & \text { for } \mathrm{t} \notin [t_{a}, t_{a'}] \\
y_{t} + {a_{a}} & \text { for } \mathrm{t} \in [t_{a}, t_{a'}]
\end{array}\right.
\label{eq:attackaa} 
\end{equation}


\subsubsection{The ramping attack}
The ramping attack vector $a_r$ is gradually modified the actual measurement with time during attack which can be modeled as below Eq.(\ref{eq:attackra}): 

\begin{equation}
y^{a}_{t}=\left\{\begin{array}{ll}
y_{t} & \text { for } \mathrm{t} \notin [t_{a}, t_{a'}] \\
y_{t} + {a_{r}} t & \text { for } \mathrm{t} \in [t_{a}, t_{a'}]
\end{array}\right.
\label{eq:attackra} 
\end{equation}

Other than the attack model, there are two ways to inject the signal of such attacks. The constant signal can is considered as one time attack which the attacker only implement the attack in a specific time period (e.g., $[t_{a}, t_{a'}]$). Another one is called periodic signal which the attacker inject the malicious vectors repeatedly within a period $T$ (e.g., $ [T+t_{a}, T+ t_{a'}]$). 


More specifically, When the information transferred between the nodes through the cyber layer, the active power and reactive power of the neighboring converters can be manipulated. The primary droop control scheme will be deceived since the malicious measurements are taken. Therefore, the system frequency and voltage stability are disturbed directly via droop control with the incorrect measurement.   

% We assume that the adversary only can compromise the communication information while the state variable collected from itself is secured since it does not involve any communication process. 


\subsection{Attack impact}

% When the information transferred between the nodes through the cyber layer, the active power and reactive power of the neighboring converters can be manipulated. The primary droop control scheme will be deceived since the malicious measurements are taken. Therefore, the system frequency and voltage stability are disturbed directly via droop control with the incorrect measurement.   

% We assume that the adversary only can compromise the communication information (e.g., $P_{Gi}, Q_{Gi}$) while the measurement collected from itself is secured since it does not involve any communication process (e.g., $P_{Gi}, Q_{Gi}$). In order to maintain stealth, it is assumed that the attacker compromises targeted converters (can be one or all of them) only one time at time $t$. T


% It can be formulated as in Eq.(\ref{eq:attackpq}), where $P_{m}^{a}$ and $Q_{G}^{a}$ are the altered active power and reactive reference power of one converters at time $t$.   
 

 
%  \begin{equation}
% \left[\begin{array}{c}
% P_{G}^{a} (t) \\
% Q_{G}^{a} (t)
% \end{array}\right]=\left[\begin{array}{c}
% P_{G} (t)\\
% Q_{G} (t)
% \end{array}\right]+\left[\begin{array}{l}
% x^{a}_{P} (t)\\
% x^{a}_{Q} (t)
% \end{array}\right]
%  \label{eq:attackpq}   
% \end{equation}
 

% The reference active power of the converters $i$ under attack at time $t+h$ ($h$ refers to the time step) can be calculated through the following Eq.(\ref{eq:attackp}), where $P_{G i}^{a}(t)$ and $P_{G j}^{a}(t)$ are the reference active power of the converters $i$ and $j$ at previous time step $t$ respectively, $w_{i j}$ is the weight factor which presents the importance of the information collected from node $i$ to node $j$. 

% \begin{equation}
% \begin{aligned}
% P_{G i}^{a}(t+h)&=P_{G i}^{a}(t)+\sum_{j \in V} w_{j i}\left[P_{G j}^{a}(t)-P_{G i}^{a}(t)\right] \\
% &= (1-\sum_{j \in V} w_{j i}) \cdot P_{G i}^{a}(t) + \sum_{j \in V} w_{j i} \cdot P_{j G}^{a}(t) \\
% &=  w_{j j} \cdot P_{G i}^{a}(t) + \sum_{j \in V} w_{j i} \cdot P_{G j}^{a}(t) \\
% &=\sum_{j = 1 }^{n} w_{j i} \cdot P_{G j}^{a}(t) 
% \end{aligned}
% \label{eq:attackp}  
% \end{equation}

% w_{m m L}(k)=1-\sum_{j \in \mathcal{N}_{m}(k)} w_{m j L}

The active power reference under attack at time $t+h$ can be written as Eq.(\ref{eq:Tg1}):

\begin{equation}
\begin{aligned}
\mathbf{P}^{a}_{G}(t+h)= \mathbf{w}  \mathbf{P}_{G}(t)& + \mathbf{w} [x^{a_1}(t)...x^{a_n}(t)]^{T}\\
&- diag[w_{ii}][x^{a_1}(t)...x^{a_n}(t)]^{T} \\
=\mathbf{w} \mathbf{P}_{G}(t)& + \mathbf{w'} [x^{a_1}(t)...x^{a_n}(t)]^{T}
\end{aligned}
\label{eq:Tg1}
\end{equation}


% \begin{multline}
% \mathbf{P}^{a}_{G}(t+h)&= \mathbf{w} \mathbf{P}(t) + \mathbf{w} [X^{a_1}(t)...X^{a_n}(t)]^{T}\\
% - diag[w_{ii}[X^{a_1}(t)...X^{a_n}(t)]^{T} ]\\
% &=\mathbf{w} \mathbf{P}(t) + \mathbf{w'} [X^{a_1}(t)...X^{a_n}(t)]^{T}
% \label{eq:q_learning}
% \end{multline}



{where the weighted factor $\mathbf{w}$ is the weight factor which presents the importance of the information collected which considered as a convex weight \cite{simpson2015secondary} $w_{ji} = a_{ji}/ \sum^{x}_{k=1}a_{ki} $ with $\sum^{x}_{k=1} w_{ki}=1$, $\mathbf{P}_{G}(t)$ refers to the actual active power reference without attack, $\mathbf{w'}= \mathbf{w}-diag({w_{ii}})$ eliminated all the unattackable local measurements. This general model can be applied to any kind of attack scenario. For example, when the communication disruption is observed between LC1 and LC2 at time $t$, the attack vectors in the active and reactive power can be modeled as $[x^{a1}_{P}, x^{a2}_{P} ...0]^{T}$ and $[x^{a1}_{Q}, x^{a2}_{Q} ...0]$ with a direct impact on their transferred information at time $t+h$.}


{Although only the targeted nodes is affected at time $t+h$, it gradually expand to more nodes when the information interchanges through the cyber network. At time $t+mh$, the active power reference can be represented as:}  


\begin{equation}
\begin{array}{l}
\mathbf{P}^{a}_{G}(t+mh)= \mathbf{w^{m-1}} \mathbf{P}^{a}_{G}(t+h)
\end{array}
\label{eq:Tg2}
\end{equation}


{Substitution of Eq. (\ref{eq:Tg1}) into Eq. (\ref{eq:Tg2}) leads to Eq (\ref{eq:Tg3}), which unveils the impact of the attack at time $t$ to the active power reference at time $t+mh$, where $\mathbf{w^{m}} \mathbf{P}_{G}(t)$ refers to the actual active power reference without attack and latter item represents the attack impact.  }



\begin{equation}
\begin{array}{l}
\mathbf{P}^{a}_{G}(t+mh)= \mathbf{w^{m}} \mathbf{P}_{G}(t)+ \mathbf{w^{m-1}} \mathbf{w'} [x^{a_1}(t)...x^{a_n}(t)]^{T}
\end{array}
\label{eq:Tg3}
\end{equation}




% Similarly, the compromised reactive power can be represented as:  
% \begin{equation}
% \begin{aligned}
% Q_{G i}^{a}(t+h)=\sum_{j = 1 }^{n} w_{j i} \cdot Q_{G j}^{a}(t) 
% \end{aligned}
% \label{eq:attackq}  
% \end{equation}


Similarly, the direct impact on the reactive power reference when the communication is compromised at time $t$ can be represented in Eq.(\ref{eq:TQ1}), the compromised reactive power reference can be calculated as shown in Eq.(\ref{eq:TQ2}) and the impact of the attack at time $t$ on the reactive power reference can be written as Eq.(\ref{eq:TQ3}) .

\begin{equation}
\begin{aligned}
\mathbf{Q}^{a}_{G}(t+h)= \mathbf{w}  \mathbf{Q}_{G}(t)& + \mathbf{w} [x^{a_1}(t)...x^{a_n}(t)]^{T}\\
&- diag[w_{ii}[x^{a_1}(t)...x^{a_n}(t)]^{T} ]\\
=\mathbf{w} \mathbf{Q}_{G}(t)& + \mathbf{w'} [x^{a_1}(t)...x^{a_n}(t)]^{T}
\end{aligned}
\label{eq:TQ1}
\end{equation}

\begin{equation}
\begin{array}{l}
\mathbf{Q}^{a}_{G}(t+mh)= \mathbf{w^{m-1}} \mathbf{Q}^{a}_{G}(t+h)
\end{array}
\label{eq:TQ2}
\end{equation}

\begin{equation}
\begin{array}{l}
\mathbf{Q}^{a}_{G}(t+mh)= \mathbf{w^{m}} \mathbf{Q}_{G}(t)+ \mathbf{w^{m-1}} \mathbf{w'} [X^{a_1}(t)...X^{a_n}(t)]^{T}
\end{array}
\label{eq:TQ3}
\end{equation}


% The reference active power of the converters under attack at time $t+h$ ($h$ refers to the time step) can be calculated through the following Eq.(\ref{eq:Tg}), where $P_{G i}^{a}(t)$ and $P_{G j}^{a}(t)$ are the reference active power of the converters $i$ and $j$ at previous time step $t$ respectively,





When the attacker targeted to more nodes in the grid, the total active power generation will be changed as shown in Eq.(\ref{eq:Tgeneration}) with compromised number of $cn$ converters (out of $D$). 


\begin{equation}
\begin{aligned}
P_{TG}^{a} = \sum^{cn}_{\alpha =1}P_{G i}^{a}+ \sum^{D-cn}_{\beta =1}P_{G i}\\
Q_{TG}^{a} = \sum^{cn}_{{\alpha =1}}Q_{G i}^{a}+ \sum^{D-cn}_{{\beta=1}}Q_{G i}
\end{aligned}
\label{eq:Tgeneration}
\end{equation}



% The total active power supplied by the DGs ($P_{G} = \sum^{x}_{P_{G=1}}p_{G}$) is the summation of all the power generated from the DG units, where $p_{G}$ refers to the power supply from one inverter. 

In order to maintain a normal operation, the demand should be less than the total generated power $P_{TG} \geq  P_L$. The total power demand ($P_L$) in the system is demonstrated in Eq.(\ref{eq:Tload}), where $p_L$ is the power demand of one load and $P_{loss}$ represents the total losses.

\begin{equation}
 P_{L} = \sum_{P_{L}=1}^{y} p_{L} + P_{loss}
\label{eq:Tload}
\end{equation}


However, the power balance can not hold when the converter is under attacked since the droop control is deceived to adjust the output of the converter. Thus, in order to verify the stability of the MG, a observation of the frequency and voltage is needed. 


\end{comment}



% \newpage

% Therefore, the control input under attack ($u^{a}_{t}$) is defined as , and the compromised measurements ($y^{a}$) will be  $  y_{a}(k+1) = C\big(x(k+1) + B\Delta u(k)\big) + e(k+1)$.


% \begin{equation}
% \begin{aligned}
% {x}&=\left[{\delta}, {f}, P, Q, P_{\text {ref}} ,V\right]\\
% {u}&=\left[{f_{ref}}\right]^{T}
% \label{eq:xandu}
% \end{aligned}
% \end{equation}


% Thus, the altered control input ($f_{ref}^{a}$) can be written as $f^{a}_{ref} = f_{ref} + m \cdot \Delta {P}$, where $f_{ref}$ is the nominal frequency reference, $m$ is the droop coefficients of the compromised inverter, and $ \Delta P$ is the difference between the active power output $ P$ with its active power reference $P_{\text {ref}}$. 






% % \begin{equation}
% %  f_{i}^{a} = f + m_{i} \cdot \Delta {P}\\
% % \end{equation}


% % \begin{equation}
% % \begin{aligned}
% % &\boldsymbol{x}=\left[\boldsymbol{\delta}, \boldsymbol{\omega}, \mathbf{i}_{d}, \mathbf{i}_{q}, \mathbf{i}_{\text {dref }}, \mathbf{i}_{\text {qref }}, \mathbf{u}_{d}, \mathbf{u}_{q}, P, Q, P_{\text {ref }}, \mathbf{V}_{d}, \mathbf{V}_{q},\right.\\
% % &\left.\mathbf{i}_{\boldsymbol{x}}, \mathbf{i}_{\boldsymbol{y}}, \mathbf{V}_{\boldsymbol{x}}, \mathbf{V}_{\boldsymbol{y}}\right]^{T}, \boldsymbol{r}_{0}=\left[\boldsymbol{\omega}_{0}\right]^{T}, \text { and the system matrix } E \text { is }
% % \end{aligned}
% % \end{equation}



% % \begin{equation}
% % \begin{aligned}
% % f_{i} &= f_{set} + m_{i} \cdot \Delta {P}\\
% % % v_{i} &= v_{set} + v_{i} \cdot \Delta {Q}\\
% % \end{aligned}
% % \label{eq:12}
% % \end{equation}






% Due to the frequency stability of the power grid determined by the power balance, the total power demand and power generation are modeled as shown in Eq.(\ref{eq:balance}), where there are number of $m$ PV and number of $n$ load in the system. If the micro-grid operates in a grid-connected model which means a connection with the central grid (e.g., Utility), thus the amount of power $P_{G}$ is provided to the micro-grid. Otherwise, it requires a power balance between the power generation from all PVs $(\sum_{x=0}^{m} P_{PV}(k))$ and the power consumption of all loads ($\sum_{y=0}^{n} P_{L}(k)$), where $P_{G}=0$.


% \begin{equation}
% \label{eq:balance}
%     P_{G}(k) + \sum_{x=0}^{m} P_{PV}(k) = \sum_{y=0}^{n} P_{L}(k)
% \end{equation}


